Tokenization and Morphological Fidelity in Uralic NLP: A Cross-Lingual Evaluation

Subword tokenization critically affects Natural Language Processing (NLP) performance, yet its behavior in morphologically rich and low-resource language families remains under-explored. This study systematically compares three subword paradigms -- Byte Pair Encoding (BPE), Overlap BPE (OBPE), and Unigram Language Model -- across six Uralic languages with varying resource availability and typological diversity. Using part-of-speech (POS) tagging as a controlled downstream task, we show that OBPE consistently achieves stronger morphological alignment and higher tagging accuracy than conventional methods, particularly within the Latin-script group. These gains arise from reduced fragmentation in open-class categories and a better balance across the frequency spectrum. Transfer efficacy further depends on the downstream tagging architecture, interacting with both training volume and genealogical proximity. Taken together, these findings highlight that morphology-sensitive tokenization is not merely a preprocessing choice but a decisive factor in enabling effective cross-lingual transfer for agglutinative, low-resource languages.

==> sections/downstream.tex <==
\section{Performance on Downstream Task}
\label{sec:downstream}


\subsection{POS Tagging}
POS tagging provides a controlled and interpretable downstream task for evaluating subword tokenization methods in morphologically rich Uralic languages. These languages exhibit extensive agglutinative morphology, productive derivation, vowel harmony, consonant gradation, and complex case systems \citep{}.

To isolate the effect of tokenization on morphosyntactic learning, we adopt two well-established POS tagging architectures with complementary modeling properties: a BiLSTM–CRF model \citep{lample-etal-2016-neural, ma-hovy-2016-end} and the Flair contextual string embeddings framework \citep{akbik2018coling, akbik2019flair}.
BiLSTM–CRF represents a classical but robust sequence-labeling architecture that remains competitive on many morphologically complex languages. Importantly, it relies solely on local contextualized representations learned from the input sequence, making it highly sensitive to subword segmentation quality and thus well suited for controlled tokenization comparisons. This model offers a clean test bed: subword embeddings are learned from scratch, and the CRF decoding layer encourages consistent POS sequences without relying on large pre-trained language models.

Flair, in contrast, provides character-level contextual string embeddings that capture long-range dependencies and subword-internal regularities. Uralic languages own pervasive morphophonology. For example, consonant gradation in Finnish and Sámi, or agglutinative suffix chains in Hungarian. the ability to represent morphology at the character level is particularly valuable. At the same time, Flair still treats token boundaries as meaningful segmentation units, meaning that tokenization influences how character sequences are grouped and contextualized. 

Evaluation is conducted on the original UD sets for target languages. To assess the downstream impact of tokenization on part-of-speech (POS) tagging, we employ Accuracy and Macro-F1 scores, complemented by a fine-grained analysis of error distribution. While accuracy provides a straightforward measure of correctly predicted tags, relying solely on aggregate metrics can obscure critical model weaknesses, particularly in structurally complex and low-resource settings \citep{mompelat-2025-simple}. Therefore, we incorporate Macro-F1, which calculates metrics for each class independently before averaging, thereby ensuring that performance on under-represented morphological categories is weighted equally to dominant classes like nouns or verbs. Furthermore, because aggregate metrics can obscure specific model weaknesses, we examine the error distribution across morphological categories; following the methodology of \citet{mompelat-2025-simple}, this granular analysis allows us to identify specific linguistic confusion patterns and determine if certain tokenization strategies systematically fail to resolve ambiguities in complex or low-frequency morphological tags.

\subsubsection{Correlation Analysis}

To complement the downstream POS tagging results, we conduct a correlation-based analysis to examine whether the relative effectiveness of OBPE is systematically associated with language-level properties, in particular resource availability, genealogical relatedness, and script alignment. To complement the downstream POS tagging results, we conduct a correlation-based analysis to examine whether the relative effectiveness of OBPE is systematically associated with language-level properties, in particular resource availability, genealogical relatedness, and script alignment. 

For each language and tokenizer configuration, we consider the two evaluation metrics reported in the POS tagging experiments: Accuracy and Macro$F1$.

Language characteristics are derived from the experimental setup and dataset statistics (Table~\ref{tab:language_info}). We consider:
\textbf{(i)} training data size, measured as the number of training sentences;
\textbf{(ii)} resource availability, treated as an ordinal variable (HIGH, MID, LOW, UNDER);
\textbf{(iii)} genealogical relatedness, distinguishing Uralic–Uralic transfer from non-genealogical transfer; and
\textbf{(iv)} script alignment, distinguishing Latin script and Cyrillic script pairings.

For each language–tokenizer configuration, we extract two evaluation metrics from the POS tagging experiments: Accuracy and Macro$F1$. Accuracy reflects overall tagging correctness and is dominated by frequent POS categories. Macro$F1$ assigns equal weight to all tags and is therefore more sensitive to segmentation errors affecting infrequent and morphologically marked categories.

Given the small sample size and the ordinal nature of several variables, we employ Spearman’s rank correlation coefficient ($\rho$) to assess monotonic associations between tokenizer gains and language-level factors. The correlations between the performance gains of OBPE ($\Delta \text{Acc}$, $\Delta F1$) and each variable of the language-level are calculated independently. No assumptions of linearity or normality are made.

This analysis is deliberately restricted to high-level associations and does not attempt to disentangle causal effects. In particular, it does not control for architectural or optimization factors, which are held constant across experiments. Instead, the correlation analysis serves to evaluate whether OBPE’s relative advantages are consistently aligned with genealogical proximity and resource conditions, and whether shared script alone is sufficient to yield comparable gains in the absence of language family relatedness.




\begin{table*}
    \centering
    \small
    \renewcommand{\arraystretch}{1.2} 
    
    \begin{tabular}{ll|cccc}
        \hline
        & & \multicolumn{2}{c}{\textbf{BiLSTM--CRF}} & \multicolumn{2}{c}{\textbf{Flair}} \\
        
        \cline{3-6} 
        
        \textbf{Language} & \textbf{Tokenizer} 
        & \textbf{Acc} & \textbf{Mac F1}
        & \textbf{Acc} & \textbf{Mac F1}  \\ 
        \hline
        Hungarian 
            & BPE     & 0.8096 & 0.7013 & 0.9509 & 0.793 \\
            & Unigram & 0.7840 & 0.6663 & 0.9408 & 0.7651\\
            & OBPE (hu-fi)   & \textbf{0.8514} 
            & 0.7412 & 0.9581 & 0.7907   \\
            & OBPE (hu-et)   & 0.8496 
            & 0.7398 & \textbf{0.9614} & 0.7902      \\        

        \hline
        
        North Sami 
            & BPE     & 0.7749 & 0.7573 & 0.9075 & 0.805 \\
            & Unigram & 0.7830 & 0.7573 & 0.9078 & 0.7885  \\
            & OBPE (sme-fi)    & 0.8036 
            & 0.7914 & 0.9264 & 0.8164\\
            & OBPE (sme-et)   & \textbf{0.8152} 
            & 0.7850 & \textbf{0.9373}  & 0.839 \\
        \hline

        Komi-Zyrian 
            & BPE     & 0.6744 & 0.4742 & 0.3941 & 0.4409 \\
            & Unigram & \textbf{0.7401} & 0.5209 & \textbf{0.9101} & 0.6367 \\
            & OBPE    & 0.7207 & 0.5022 & 0.893 & 0.5693  \\
        \hline
    \end{tabular}
    \caption{Performance comparison of BiLSTM--CRF and Flair models across 5 languages and 3 tokenizers.}
    \label{tab:pos_model_comparison}
\end{table*}


==> tabfig/acc_f1.tex <==
\begin{table}
    \centering
    \small
    \renewcommand{\arraystretch}{1.2} 
    \resizebox{\linewidth}{!}{
    % 8 Columns: Lang | Tok || BiLSTM (3 cols) || Flair (3 cols)
    \begin{tabular}{ll|cccc}
        \hline
        % --- Row 1: Model Headers ---
        % Empty first two cells, then span 'BiLSTM--CRF' over 3 cols, then 'Flair' over 3 cols
        & & \multicolumn{2}{c}{\textbf{BiLSTM--CRF}} & \multicolumn{2}{c}{\textbf{Flair}} \\
        
        % Draw a line only under the model names (columns 3 to 8)
        \cline{3-6} 
        
        % --- Row 2: Metric Headers ---
        \textbf{src$\rightarrow$tgt} & \textbf{Tokenizer} 
        & \textit{Acc} & \textit{Mac F1}  % Metrics for BiLSTM
        & \textit{Acc} & \textit{Mac F1}  \\ % Metrics for Flair
        \hline
        %\hline
        \texttt{est} $\rightarrow$ \texttt{hun}  
            & BPE     & - & - & - & - \\
            & Unigram & - & - & - & - \\
            & \cellcolor{lightgray} OBPE    
            & \cellcolor{lightgray} - 
            & \cellcolor{lightgray} - 
            & \cellcolor{lightgray} - 
            & \cellcolor{lightgray} -  \\
        \hline
        
        \texttt{est} $\rightarrow$ \texttt{sme}  
            & BPE     & - & - & - & - \\
            & Unigram & - & - & - & - \\
            & \cellcolor{lightgray} OBPE    
            & \cellcolor{lightgray} - 
            & \cellcolor{lightgray} - 
            & \cellcolor{lightgray} - 
            & \cellcolor{lightgray} -  \\
        \hline
        
        % --- Hungarian ---
        \texttt{fin} $\rightarrow$ \texttt{hun}  
            & BPE     & 0.8096 & 0.7013 & 0.9509 & \textcolor{blue}{0.7930} \\
            & Unigram & 0.7840 & 0.6663 & 0.9408 & 0.7651\\
            
            & \cellcolor{lightgray} OBPE (hu-fi)   
            & \cellcolor{lightgray}\textcolor{blue}{0.8514} % hu_fi
            & \cellcolor{lightgray}\textcolor{blue}{0.7412} 
            & \cellcolor{lightgray} 0.9581 
            & \cellcolor{lightgray} 0.7907   \\
            %& \cellcolor{lightgray} OBPE (hu-et)   
            %& \cellcolor{lightgray} 0.8496 % hu_et
            %& \cellcolor{lightgray} 0.7398 
            %& \cellcolor{lightgray}\textcolor{blue}{0.9614} 
            %& \cellcolor{lightgray} 0.7902      \\
                   

        \hline
        
        % --- North Sami ---
        \texttt{fin} $\rightarrow$ \texttt{sme}  
            & BPE     & 0.7749 & 0.7573 & 0.9075 & 0.8050 \\
            & Unigram & 0.7830 & 0.7573 & 0.9078 & 0.7885  \\
            & \cellcolor{lightgray} OBPE (sme-fi)   
            & \cellcolor{lightgray} 0.8036 %sme_fi
            & \cellcolor{lightgray} \textcolor{blue}{0.7914}
            & \cellcolor{lightgray} 0.9264 
            & \cellcolor{lightgray} 0.8164 \\
            %& \cellcolor{lightgray} OBPE (sme-et)   
            %& \cellcolor{lightgray} \textcolor{blue}{0.8152} %sme_fi
            %& \cellcolor{lightgray} 0.7850 
            %& \cellcolor{lightgray} \textcolor{blue}{0.9373}  
            %& \cellcolor{lightgray} \textcolor{blue}{0.8390} \\
            
        \hline
        %
        % --- Komi-Zyrian ---
        \texttt{rus} $\rightarrow$ \texttt{kpv}  
            & BPE     & 0.6744 & 0.4742 & 0.3941 & 0.4409 \\
            & Unigram & \textcolor{blue}{0.7401} & \textcolor{blue}{0.5209} & \textcolor{blue}{0.9101} & \textcolor{blue}{0.6367} \\
            & \cellcolor{lightgray} OBPE    
            & \cellcolor{lightgray} 0.7207 
            & \cellcolor{lightgray} 0.5022 
            & \cellcolor{lightgray} 0.8930 
            & \cellcolor{lightgray} 0.5693  \\
        \hline
    \end{tabular}
    }
    
    \caption{Performance of tokenizers on POS tagging of two source languages (Finnish and Russian) and four target languages.}
    \label{tab:pos_model_comparison}
\end{table}
